DB-PAISA: Discovery-Based Privacy-Agile IoT Sensing+Actuation

Internet of Things (IoT) devices are becoming increasingly commonplace in numerous public and semi-private settings. Currently, most such devices lack mechanisms to facilitate their discovery by casual (nearby) users who are not owners or operators. However, these users are potentially being sensed, and/or actuated upon, by these devices, without their knowledge or consent. This naturally triggers privacy, security, and safety issues. To address this problem, some recent work explored device transparency in the IoT ecosystem. The intuitive approach is for each device to periodically and securely broadcast (announce) its presence and capabilities to all nearby users. While effective, when no new users are present, this push-based approach generates a substantial amount of unnecessary network traffic and needlessly interferes with normal device operation. In this work, we construct DB-PAISA which addresses these issues via a pull-based method, whereby devices reveal their presence and capabilities only upon explicit user request. Each device guarantees a secure timely response (even if fully compromised by malware) based on a small active Root-of-Trust (RoT). DB-PAISA requires no hardware modifications and is suitable for a range of current IoT devices. To demonstrate its feasibility and practicality, we built a fully functional and publicly available prototype. It is implemented atop a commodity MCU (NXP LCP55S69) and operates in tandem with a smartphone-based app. Using this prototype, we evaluate energy consumption and other performance factors.

==> contents/paisa_inventory_detailed.tex <==
\section{\paisaplus Variant -- \private \label{sec:inventory}}
%

\begin{figure}[t]
  \centering
  \captionsetup{justification=centering}
  \includegraphics[width=0.95\columnwidth]{img/inventory.pdf}
  \vspace{-0.3cm}
  \caption{\private Overview}
  \label{fig:inventory}
  \vspace{-0.4cm}
\end{figure}

\private has two components: \ownerdev and \iotdev. \ownerdev is the owner's device authorized to 
solicit information from a multitude of \iotdev-s in a large industrial setting.
As shown in Figure \ref{fig:inventory}, \private also has two phases: {\it Registration} and {\it Runtime}.

\noindent {\bf $\boldsymbol{\registration}$ phase} occurs prior to device deployment.
Each \iotdev is securely provisioned with (1) unique secret key (\seckey) shared with \ownerdev, 
(2) its own device information, and (3) \ownerdev's public key (\ownerpk).

\noindent {\bf $\boldsymbol{\runtime}$ phase} has three steps: \request, \response, and \receptionusr.
There are three significant differences from \pub: (1) \requestmessage is authenticated with 
\ownerdev's private key (\ownersk), (2) \responsemessage is encrypted with \seckey, and
(3) \attest takes place upon every \requestmessage.

\noindent {\em NOTE:} Due to space constraints, implementation and evaluation of \private are not present in this work.
Nonetheless, we fully implemented it at \cite{paisaplus-code}.


\subsection{\private Adversary model} \label{subsec:inventory-adv}
%
\noindent {\bf DoS attacks on \iotdev-s:}
Similar to \pub, malware \sadv can try to deplete \iotdev resources via software vulnerabilities.
However, DoS attacks from a network \sadv are more challenging to address because of costly
verification of \ownerdev's signatures in \requestmessage-s.
Potential mitigation techniques are discussed in Section \ref{subsec:discussion-dos}.

\noindent {\bf Replay attacks:}
A network-based \sadv can replay arbitrary messages to both \ownerdev and \iotdev-s.

\noindent {\bf Eavesdropping:}
A network-based \sadv can eavesdrop on all \private protocol messages to learn
individual \iotdev information and the number and types of deployed \iotdev-s.
\sadv can also attempt to link occurrences of one or more \iotdev-s.


\subsection{\private Requirements}
%
\noindent{\bf System requirements:} are the same as in \pub, except that scaling to multiple users is no longer a concern in \private.
Although \private operates in settings with large numbers of \iotdev-s, only an authorized \ownerdev can solicit information from them. 


\noindent{\bf Security requirements (beyond those of \pub):}
%
\begin{compactitem}
    \item {\it Request authentication:} \iotdev must validate each \requestmessage.
    \item {\it Response confidentiality:} \responsemessage must not leak information about \iotdev.
    \item {\it Unlinkability:} Given any two valid \responsemessage-s, the probability of determining if they were produced by the same \iotdev should be negligibly close to 50\%, for any party except \ownerdev.
\end{compactitem}
%

\subsection{\private Protocol Details} \label{subsec:inventory_detail}
In this section, we only describe the aspects of \private that differ from \pub.
Figures \ref{fig:prot-inv-reg} and \ref{fig:prot-inv-runtime} summarize \registration and \runtime phases, respectively.


\subsubsection{Registration}
%
\ownerpk, \seckey, and some metadata are securely installed for each \iotdev. However, information 
that is not deployment-dependent (such as \privatetcb, \iotdevsofthash, and peripheral configuration) 
are assumed to be securely provisioned earlier by \mfr. 
Note that, since \ownerdev is aware of all identities and types of its \iotdev-s, there is no 
longer any need for either {\bf $\boldsymbol{\devmanifest}$} or {\bf $\boldsymbol{\devmanifesturl}$}.
As a result, \mfr plays no active role in \private.
The {\bf TCB} of \private is identical to that of \pub.


\begin{figure}[t]
  \centering  
  \captionsetup{justification=centering}  
  \includegraphics[height=1.8in,width=0.95\columnwidth]{img/inventory_state_machine.pdf}
  \vspace*{-.3cm}  
  \caption{\private State Machine on \iotdev}
  \label{fig:inventory_state_machine}
  \vspace*{-0.35cm}
\end{figure}


\subsubsection{Runtime} \label{subsubsec:inventory-runtime}
%
Similar to \pub, the \private \runtime phase has three steps: \request, \response, and \receptionusr.

\paragraph{\bf $\boldsymbol{\privatetcb}$ on $\boldsymbol{\iotdev}$: }
As discussed in Section \ref{subsec:inventory-adv}, DoS attacks by a network-based \sadv are out-of-scope.
Also, scalability is not an issue since only one \ownerdev is assumed.
Furthermore, because \ownerdev's requests are expected to be much less frequent 
than \usrdev's requests in \pub, \attest is performed on the fly upon each \ownerdev's request.

Figure \ref{fig:inventory_state_machine} shows four state machines of \iotdev:

\noindent{\bf (a) $\boldsymbol{\wait}$:}
The only transition is switching to $\boldsymbol{\verifystep}$ when \requestmessage is received.

\noindent{\bf (b) $\boldsymbol{\verifystep}$:}
\iotdev verifies \requestmessage with \ownerpk.
If verification succeeds, it transitions to $\boldsymbol{\attest}$.
Otherwise, it discards \requestmessage and returns to $\boldsymbol{\wait}$.

\noindent{\bf (c) $\boldsymbol{\attest}$:}
\iotdev computes \attestresult and transitions to $\boldsymbol{\gen}$.
Note that \iotdev need not compute attestation time because \attest occurs with every \requestmessage, thus $\attestreport := [\attestresult]$.


\noindent{\bf (d) $\boldsymbol{\gen}$:}
\iotdev encrypts \noncevalue{\owner}{} (\ownerdev's nonce in \requestmessage), device information (e.g., \iotdevid, \iotdev type, 
\iotdevsoft version), and \attestreport with \seckey, i.e., $\encvalue{\resp} := \encfunc(\seckey, \noncevalue{\owner}{}||\attestreport||\text{device information})$, where \encfunc\ is an encryption operation.
It composes \responsemessage containing an authentication tag, e.g., using AES-CCM/GCM.
Since \responsemessage is encrypted, multiple \responsemessage-s from the same \iotdev are
unlinkable as long as: (1) \seckey is not leaked, (2) \seckey is sufficiently long and randomly
chosen, and (3) the underlying symmetric encryption algorithm is secure.
%
However, we acknowledge that address information in packet headers of \responsemessage-s 
can be used to track \iotdev. We discuss how to address this problem in 
Appendix \ref{subsection:appendix-discussion}.


\paragraph{\bf $\boldsymbol{\private}$ app on $\boldsymbol{\ownerdev}$: }
There are two steps on \ownerdev: \request and \receptionusr.

\noindent{\bf \request:} \ownerdev signs \noncevalue{\owner}{} with \ownersk \ and broadcasts \requestmessage, containing \noncevalue{\owner}{} and the signature (\sigvalue{\req}).
After sending \requestmessage, it starts a scan to receive \responsemessage-s from potential nearby \iotdev-s.

\noindent{\bf \receptionusr:}
Upon receiving \responsemessage, \ownerdev retrieves the corresponding \seckey in brute-force attempts, i.e., it attempts to decrypt \requestmessage with all \seckey-s.
This demands O($n$) computations on \ownerdev, where $n$ is the number of \iotdev.
Its overhead and alternative approaches are discussed in Section \ref{sec:discussion-key-retrieval}.
After retrieving \seckey, it decrypts it with the \seckey, and finally, details are displayed on \ownerdev.

\subsection{Discussion} \label{subsection:appendix-discussion}
\noindent {\bf $\boldsymbol{\requestmessage}$ DoS Mitigation:}
Mitigating DoS attacks in \private is more challenging. The lazy-response technique used in \pub is
unsuitable for \private because each \requestmessage requires individual verification and response.
One radical approach is to skip verification of \requestmessage-s altogether.
This way, \iotdev inundated with \requestmessage-s would generate as many 
\responsemessage-s. However, symmetric encryption of \responsemessage-s is much
less expensive than signature verification of \requestmessage-s.
Also, lack of \requestmessage authentication would allow a network-based \sadv to generate
fake \requestmessage-s and harvest replies.
Although \sadv would not be able to track individual \iotdev-s, it can easily learn {\em the number} of nearby \iotdev-s.

Another alternative is using Lamport's hash chains \cite{lamport1981} to authenticate \requestmessage-s.
While inexpensive, hash chains prompt well-known synchronization issues, plus the need to support a separate
(and robust) hash chain renewal mechanism.

\noindent {\bf $\boldsymbol{\iotdev}$ Unlinkability of $\boldsymbol{\responsemessage}$-s:}
%
As mentioned earlier, if a network-based \sadv learns that multiple \responsemessage-s 
are emitted by the same \iotdev, it can effectively track that it.

As discussed in Section \ref{sec:inventory}, all fields in \responsemessage 
are encrypted and \seckey is presumably never leaked, sufficiently long (bit-wise), and
randomly selected. Also, the underlying symmetric encryption algorithm is secure.
Furthermore, all \responsemessage-s must be of uniform size, regardless of the type/model
of the responding \iotdev. Therefore, we can rule out linkability based on analysis of 
\responsemessage payloads.

However, the BLE packet header format includes certain static fields, such as the MAC address and UUID.
\iotdev can be trivially tracked by observing these fields in multiple BLE packets \cite{bello2019privacy}.
Fortunately, BLE supports MAC address randomization to prevent tracking \cite{ludant2021linking}.
Randomization can be done periodically (e.g., daily or hourly) or based on an event (e.g., per packet).
Although this raises some performance issues (such as connection un-pairing, 
MAC address change overhead), \iotdev in \private can randomize the MAC address per \responsemessage.
We believe this is acceptable since \ownerdev is expected to issue requests relatively infrequently. 
Finally, to prevent UUID-based tracking, we insert a random UUID into every \requestmessage header.

==> img/embedfont <==
gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX \
-dPDFSETTINGS=/prepress -sOutputFile=$1_embed -f $1 \
-c quit

